Next-to-Leading Order Gamma Gamma + 2-Jet Production at the LHC

We present next-to-leading order QCD predictions for cross sections and for a comprehensive set of distributions in diphoton + 2-jet production at the Large Hadron Collider. We consider the contributions from loop amplitudes for two photons and four gluons, but we neglect top quarks. We use BlackHat together with SHERPA to carry out the computation. We use a Frixione cone isolation for the photons. We study standard sets of cuts on the jets and the photons, and also sets of cuts appropriate for studying backgrounds to Higgs-boson production via vector-boson fusion.

==> tables/total.tex <==
BASIC &~$2.678(0.003)^{+0.808}_{-0.577}$~&~$3.23(0.03)^{+0.31}_{-0.36}$~&~$0.0509(0.0007)$~\\ \hline
BASICVBF &~$0.1398(0.0003)^{+0.0541}_{-0.0359}$~&~$0.159(0.002)^{+0.016}_{-0.021}$~&~$0.004(0.001)$~\\ \hline
ATLAS &~$0.0886(0.0005)^{+0.0264}_{-0.0189}$~&~$0.099(0.002)^{+0.007}_{-0.010}$~&~$0.0
0157(0.00003)$~\\ \hline
ATLASVBF &~$0.00392(0.00004)^{+0.00153}_{-0.00101}$~&~$0.0046(0.0001)^{+0.0006}_{-0.0006}$~&~$0.000089(0.000004)$~\\ \hline

